BEM: Balanced and Entropy-based Mix for Long-Tailed Semi-Supervised Learning

Data mixing methods play a crucial role in semi-supervised learning (SSL), but their application is unexplored in long-tailed semi-supervised learning (LTSSL). The primary reason is that the in-batch mixing manner fails to address class imbalance. Furthermore, existing LTSSL methods mainly focus on re-balancing data quantity but ignore class-wise uncertainty, which is also vital for class balance. For instance, some classes with sufficient samples might still exhibit high uncertainty due to indistinguishable features. To this end, this paper introduces the Balanced and Entropy-based Mix (BEM), a pioneering mixing approach to re-balance the class distribution of both data quantity and uncertainty. Specifically, we first propose a class balanced mix bank to store data of each class for mixing. This bank samples data based on the estimated quantity distribution, thus re-balancing data quantity. Then, we present an entropy-based learning approach to re-balance class-wise uncertainty, including entropy-based sampling strategy, entropy-based selection module, and entropy-based class balanced loss. Our BEM first leverages data mixing for improving LTSSL, and it can also serve as a complement to the existing re-balancing methods. Experimental results show that BEM significantly enhances various LTSSL frameworks and achieves state-of-the-art performances across multiple benchmarks.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/tab1.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Require:}}
\begin{algorithm}
\caption{Balanced and entropy-based mix (BEM)}
\begin{algorithmic}[1]
% \input{}
\REQUIRE Labeled dataset $D_l$ and unlabeled dataset $D_u$, model $f$, class prior of labeled dataset $\pi$, estimated unlabeled dataset class distribution $\pi_{est}$, entropy selection
threshold $\tau_e$, balanced parameter $\alpha$, number of iterations in each epoch $K$, .
\ENSURE Weak augmentation $A_w$ and strong augmentation $A_s$
% \STATE Define some variabless
\FOR{$k=1$ to $K$}
\STATE $\{(x_i^{(l)}, y_i^{(l)})\}_{i=0}^{B-1} \gets$ Sample a batch of labeled data
\STATE $\{x_i^{(u)}\}_{j=0}^{B-1} \gets$ Sample a batch of unlabeled data
% \STATE # 
\STATE $q(x_j^{(u)}) \gets \arg \max f(A_w(x_j^{(u)}))$ 
\STATE \textbf{\{Update variables\}}
\STATE Update estimated class distribution $\pi_{est}$ based on  pseudo-labels $q(x_j^{(u)})$ according to Equ. (2) and (3)
\STATE Update class-wise entropy $e_c$ based on $f(A_w(x_j^{(u)}))$ and $f(A_w(x_i^{(l)})))$ according to Equ. (6) and (7)
\STATE Update sampling probability $\hat{s_c}$ according to Equ. (6) and (7)
\STATE Update instance-wise entropy $e$ and entropy selection threshold $\tau_e$  according to Equ. (10) and (7)
\STATE Update $M_{high}$ and $M_{low}$ according to Equ. (11) and (12)
% \STATE # 
\STATE \textbf{\{Sampling\}}
\STATE $\{(m_i^{(l)}, y_i^{(m)})\}_{i=0}^{B-1} \gets$ Sample a batch of labeled data from mix bank following $\hat{s_c}$
\STATE $\{m_i^{(u)}\}_{j=0}^{B-1} \gets$ Sample a batch of unlabeled data from mix bank following $\hat{s_c}$
\STATE \textbf{\{CamMix\}}
\STATE $\hat{x}_i^{(u)} \gets$ CamMix($x_i^{(u)},  m_i^{(l)}$) according to $M_{high}$
\STATE $\hat{x}_j^{(u)} \gets$   CamMix($x_j^{(u)},  m_j^{(u)}$) according to $M_{low}$
\STATE Update $\lambda$ according to the average of the area of mixed data
\STATE Generate sample masks $M$
\STATE \textbf{\{Compute losses\}}
\STATE $L_{l} \gets \sum_{i=0}^{B-1} l(f(x_i^{(l)}, y_i{(l)}))$
\STATE $L_{u}^{high} \gets \sum_{j=0}^{B-1} M(x_j^{(u)}) M_{high}(x_j^{(u)}) l(f(\hat{x}_j^{(u)}, q(x_j^{(u)})))$
\STATE $L_{u}^{low} \gets \sum_{j=0}^{B-1} M(x_j^{(u)}) M_{low}(x_j^{(u)}) l(f(\hat{x}_j^{(u)}, q(x_j^{(u)})))$
\STATE $L_{u^\prime}^{high} \gets \sum_{j=0}^{B-1} M(x_j^{(u)}) M_{high}(x_j^{(u)}) l(f(\hat{x}_j^{(u)}, y_i^{(m)}))$
\STATE $L_{u^\prime}^{low} \gets \sum_{j=0}^{B-1} M(x_j^{(u)}) M_{low}(x_j^{(u)}) l(f(\hat{x}_j^{(u)}, q(m_j^{(u)})))$
\STATE $L = L_{l} + \lambda( L_{u}^{high}+L_{u}^{low})+ (1-\lambda)(L_{u^\prime}^{high}+L_{u^\prime}^{low})$
\STATE Update $f$ based on $\nabla L$ using SGD
\ENDFOR
\RETURN Some results
\end{algorithmic}
\end{algorithm}
